A Comprehensive Analytical Survey on Unsupervised and Semi-Supervised Graph Representation Learning Methods

Graph representation learning is a fast-growing field where one of the main objectives is to generate meaningful representations of graphs in lower-dimensional spaces. The learned embeddings have been successfully applied to perform various prediction tasks, such as link prediction, node classification, clustering, and visualization. The collective effort of the graph learning community has delivered hundreds of methods, but no single method excels under all evaluation metrics such as prediction accuracy, running time, scalability, etc. This survey aims to evaluate all major classes of graph embedding methods by considering algorithmic variations, parameter selections, scalability, hardware and software platforms, downstream ML tasks, and diverse datasets. We organized graph embedding techniques using a taxonomy that includes methods from manual feature engineering, matrix factorization, shallow neural networks, and deep graph convolutional networks. We evaluated these classes of algorithms for node classification, link prediction, clustering, and visualization tasks using widely used benchmark graphs. We designed our experiments on top of PyTorch Geometric and DGL libraries and run experiments on different multicore CPU and GPU platforms. We rigorously scrutinize the performance of embedding methods under various performance metrics and summarize the results. Thus, this paper may serve as a comparative guide to help users select methods that are most suitable for their tasks.

==> trash.tex <==
\section{Proposed Method}
\label{sec:proposedmethod}

\subsection{Problem Formulation}
The graph embedding problem deals with the challenge of maintaining similar structural information to the original graph in the embedding space. Thus, the neighboring vertices will have a similar embedding than non-neighboring vertices. Using the similarity distribution function, we can define the likelihood of a vertex $u$ with respect to all other vertices in the graph as follows:

\begin{equation}
\label{eqn:likelihood}
    L_u = \prod_{\mathclap{v\in N_k(u)}}\sigma(z_u, z_v)^{w_{u,v}} \prod_{\mathclap{v'\notin N_k(u)}}(1-\sigma(z_u, z_{v'}))^{w'_{u,v'}}
\end{equation}

Here, $w_{u,v}$ is the weight of $k$-hope neighboring vertices $u$ and $v$, and $w'_{u,v'}$ is the weight of non-neighboring vertices. For simplicity, assuming $w_{u,v}=w'_{u,v'}=1$, Equation \ref{eqn:likelihood} can be approximated by log-likelihood. So, we can define the loss function as the negative log-likelihood using the following equation:

\begin{equation}
\label{eqn:logloss}
    \mathcal{L}_u \approx -\sum_{\mathclap{v\in N_k(u)}}\log \sigma(z_u, z_v) - \sum_{\mathclap{v'\notin N_k(u)}}\log (1-\sigma(z_u, z_{v'}))
\end{equation}

We want to optimize Equation \ref{eqn:logloss} as a minimization function $\sum_{u\in V}\mathcal{L}_u$ using a Stochastic Gradient Descent (SGD) based approach. We formulate the optimization task in terms of a spring-electrical model of force-directed graph drawing where two types of forces are calculated based on the connectivity of vertices, namely, an \emph{attractive} force when two vertices are connected by an edge and a \emph{repulsive} force when there is no connection between two vertices~\cite{fruchterman1991graph}. Without loss of generality, we compute an \emph{attractive} force upto $k$-hop neighbors. We can use any similarity distribution function in our force-directed model, two of which are discussed in the following:

\subsubsection{Sigmoid function}
Our first similarity distribution function is sigmoid, which have been widely used in graph embedding problem \cite{perozzi2014deepwalk,grover2016node2vec,tsitsulin2018verse}. Putting the value of $\sigma(z_u, z_v) = \frac{1}{1+e^{-z_u.z_v}}$ in Equation \ref{eqn:logloss}, we get the following loss function:

\begin{equation}
\label{eqn:sigmoidloglikelihood}
    \mathcal{L}_u \approx \sum_{\mathclap{v\in N_k(u)}}\log(1+e^{-z_u.z_v}) - \sum_{\mathclap{v'\notin N_k(u)}}\log \frac{e^{-z_u.z_{v'}}}{1+e^{-z_u.z_{v'}}}
\end{equation}

In Equation \ref{eqn:sigmoidloglikelihood}, the first part represents an \emph{attractive} force which is denoted by $f_a(u) = \sum_{v\in N_k(u)}\log(1+e^{-z_u.z_v})$ and the second part represents a \emph{repulsive} force which is denoted by $f_r(u) =\sum_{v'\notin N_k(u)}-\log \frac{e^{-z_u.{v'}}}{1+e^{-z_u.z_{v'}}}$. Thus, the combined force is treated as a loss function which can be represented as follows:

\begin{equation}
\label{eqn:combinedloss}
    \mathcal{L}_u = f_a(u) + f_r(u)
\end{equation}

To compute the gradient of Equation \ref{eqn:sigmoidloglikelihood}, we find the derivative with respect to $z_u$ as follows:

\begin{equation}
\label{eqn:faderivativesigmoid}
    \frac{\partial f_a(u)}{\partial z_u} = -\sum_{\mathclap{v\in N_k(u)}} (1-\sigma(z_u,z_v)).z_v
\end{equation}

\begin{equation}
\label{eqn:frderivativesigmoid}
   \frac{\partial f_r(u)}{\partial z_u} = \sum_{\mathclap{v\notin N_k(u)}} \sigma(z_u,z_v).z_v
\end{equation}

%Most of the existing state-of-the-art graph embedding methods optimize model based on softmax function~\cite{grover2016node2vec,perozzi2014deepwalk,tsitsulin2018verse,tang2015line}. In this paper, we choose student $t$-distribution for $\sigma$ which is used by many visualization tools such as t-SNE \cite{maaten2008visualizing}, UMAP \cite{mcinnes2018umap} and LargeVis \cite{tang2016visualizing}. Specifically, authors show in LargeVis that this distribution works better among many other probabilistic functions. Using this similar distribution, the likelihood of a vertex $u$ can be defined as following:

\subsubsection{Student's $t$-distribution}
Our second similarity function is $t$-distribution which has been found effective in high-dimensional data visualization~\cite{maaten2008visualizing,mcinnes2018umap}. Note that if we use one degree of freedom in $t$-distribution, it will approximate a standard Cauchy distribution \cite{luo2011cauchy}. Putting the value of $\sigma(z_u, z_v) = \frac{1}{1+t^2}$, where $t = \parallel z_u - z_v\parallel$, in Equation \ref{eqn:logloss}, we get the following:
\begin{equation}
\label{eqn:tdistloss}
    \mathcal{L}_u = \sum_{\mathclap{v\in N_k(u)}}\log(1+t^2) - \sum_{\mathclap{v'\notin N_k(u)}}\log \frac{t^2}{1+t^2}
    %\mathcal{L}_u = \sum_{\mathclap{v\in N_k(u)}}\log(1+(z_u - z_v)^2) - \sum_{\mathclap{v'\notin N_k(u)}}\log \frac{(z_u-z_v)^2}{1+(z_u - z_v)^2}
\end{equation}

Now, we can compute the gradient in a similar way to the sigmoid function. Specifically, we get the gradient of the \emph{attractive} and \emph{repulsive} forces as follows: 

\begin{equation}
\label{eqn:fatgrad}
    \frac{\partial f_a(u)}{\partial z_u} = \frac{\partial f_a(u)}{\partial t} \frac{\partial t}{\partial z_u} = \sum_{\mathclap{v\in N_k(u)}} \frac{2t}{1+t^2}
    %\frac{\partial f_a(u)}{\partial z_u} = \sum_{\mathclap{v\in N_k(u)}} \frac{2(z_u-z_v)}{1+(z_u-z_v)^2}
\end{equation}
\begin{equation}
\label{eqn:frtgrad}
    \frac{\partial f_r(u)}{\partial z_u} = \frac{\partial f_r(u)}{\partial t} \frac{\partial t}{\partial z_u}= \sum_{\mathclap{v\notin N_k(u)}} \frac{-2}{t(1+t^2)}
    %\frac{\partial f_r(u)}{\partial z_u} = \sum_{\mathclap{v\notin N_k(u)}} \frac{-2}{(z_u-z_v)(1+(z_u-z_v)^2)}
\end{equation}



\subsection{Optimization}
Once we have the gradient, we can optimize the embedding using the SGD algorithm. We will update the embedding in each iteration of the SGD for vertex $u$ as follows:

\begin{equation}
\label{eqn:update}
    z_u = z_u - \eta\frac{\partial\mathcal{L}_u}{\partial z_u}
\end{equation}
In equation \ref{eqn:update}, $\eta$ is the learning rate or step value. Note that when we use Equation \ref{eqn:sigmoidloglikelihood}, we basically optimize the embedding in a vector space, but when we use $t$-distribution, we embed the graph in a Euclidean space. Thus, we will need to multiply Equations \ref{eqn:fatgrad} and \ref{eqn:frtgrad} by a unit vector of the corresponding vertices to get the direction of movement.

In addition to Equations \ref{eqn:fatgrad} and \ref{eqn:frtgrad}, we have also employed some other popular force-directed models as gradient factors which are summarized in Table \ref{tab:diffmodels}. Most of these models are very popular in the graph drawing community and authors of ForceAtlas2 provide a precise description~\cite{jacomy2014forceatlas2}. As our method is based on a force-directed model, we name our proposed model as \toolname{}.

\begin{table}[!ht]
\centering
\caption{Different spring-electrical model with corresponding attractive and repulsive force factors.}
\begin{tabular}{|c|c|c|}

\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Spring-Electrical Model\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Attractive Force\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Repulsive Force\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}c@{}}Fruchterman Reingold\end{tabular}            & -$\parallel z_u - z_v\parallel^2$                                                                  & $1/\parallel z_u - z_v\parallel$\\ \hline
LinLog                                                                     & -$\log(1+\parallel z_u - z_v\parallel)$                                                            & $1/\parallel z_u - z_v\parallel$                                                                \\ \hline
ForceAtlas                                                                 & -$\parallel z_u - z_v\parallel$                                                                   & $1/\parallel z_u - z_v\parallel$                                                                \\ \hline
\end{tabular}
\label{tab:diffmodels}
\end{table}

\subsection{Force2Vec Algorithm}
In this section, we provide step by step discussions on the building blocks of the \toolname{} algorithm.

\subsubsection{minibatch-SGD}
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/algorithms1.pdf}
    \caption{An example showing force calculation for minibatch size 2. We start from vertex $0,1$ and consider two consecutive vertices in a minibatch shown in shaded regions. This example finishes in three steps, and each step processes a minibatch of two vertices. Green color denotes a vertex whose force is currently being computed, and Red color denotes a vertex whose coordinate is being updated.}
    \label{fig:batchforce}
\end{figure}
The straightforward implementation of SGD is helpful for optimization, but it does not facilitate the process with enough parallelization. A mini-batch version of SGD is very popular in machine learning literature as it offers more parallel works \cite{li2014efficient,rahman2020batchlayout}. In mini-batch SGD, instead of an immediate updating of the embedding to a vertex, we perform a \emph{lazy} update. This updates the embedding after processing a batch of vertices. We can describe this with an example in Fig. \ref{fig:batchforce}. In this example, the first batch consists of a set of vertices $\{0,1\}$. When we calculate forces for vertex $0$, we do not update its embedding immediately, but rather, store it for \emph{lazy} update. Similarly, when we calculate forces for vertex $1$, we do not update its embedding, but store it. After the completion of the force calculation of a batch, we update its embedding for the full batch. Note, when we calculate forces within a batch, we do not consider updated embedding of a vertex if it is a member of the current batch. When we compute the forces for next batch (e.g., $\{2,3\}$ in Fig. \ref{fig:batchforce}), we consider the updated embedding of the previous batch (i.e., $\{0,1\}$). The main advantage of this technique is that a batch can be processed in parallel, as there is no dependency, providing deterministic results, unlike asynchronous parallelization of SGD \cite{recht2011hogwild}.


% Add more text about intrinsic code etc.

%\begin{figure}
%    \centering
%    \includegraphics[width=\linewidth]{figures/decomposedmatrices.png}
%    \caption{An example of matrix decomposition for Fig. \ref{fig:batchforce} which is more friendly for SIMD vectorized operations. `A' represents attractive force and `R' represents repulsive force.}
%    \label{fig:vectorized}
%\end{figure}

\subsubsection{Algorithm}
To compute \emph{attractive} forces, we consider $k$-hope neighbors of a vertex. For \emph{repulsive} forces, we use a negative sampling approach which is widely used in the NLP domain, as well as in graph embedding problems~\cite{mikolov2013distributed,grover2016node2vec}. In negative sampling, generally, a subset of non-neighboring vertices are chosen randomly from a uniform distribution which is supposed to approximate the \emph{repulsive} force well. To make the computation faster, we choose a negative sampling for a batch instead of sampling for one vertex. We formally present \toolname{} in Algorithm \ref{algo:nsforce2vecalgo}. The algorithm starts with a random embedding $z$, with initial learning rate $\eta$, size of a minibatch as $B$ and $Max$ as the number of iterations. We choose negatives samples for a batch as shown through line 6 to line 8. Lines $9$ to $13$ represent force calculations for a batch that can be run in parallel, as there is no dependency. After that, the embedding of the batch will be updated based on the calculated forces, as shown in lines $14$ to $15$. In Algorithm \ref{algo:nsforce2vecalgo}, $\nabla f_a$ and $\nabla f_b$ represent gradients of \emph{attractive} and \emph{repulsive} forces, respectively. While calculating the gradient for the sigmoid function, we directly use Equations \ref{eqn:faderivativesigmoid} and \ref{eqn:frderivativesigmoid}, but while calculating the gradient for $t$-distribution, we use Equations \ref{eqn:fatgrad} and \ref{eqn:frtgrad} by multiplying the unit vector $\frac{z_u-z_v}{\parallel z_u -z_v \parallel}$ to get the direction of movement in $d$-dimensional Euclidean space. Note, Algorithm \ref{algo:nsforce2vecalgo} can be easily vectorized for superior performance using the SIMD instruction sets. This format of the \toolname{} model becomes useful to avoid unexpected running time bottlenecks that are commonly faced in asynchronous optimization~\cite{tang2015line,tsitsulin2018verse}.


%add more text later

The time complexity of Algorithm \ref{algo:nsforce2vecalgo} is $O(dns)$ and the space complexity is $O(m+nd)$. This complexity is the same as the sampling version of \emph{Verse} and making it helpful for processing very large graph. Though the \emph{Verse} model does not support weighted graph, our \toolname{} model support this in addition to other types of graphs. Some other algorithms for graph embedding, such as \emph{DeepWalk}, \emph{Verse} or \emph{LINE}, can be easily incorporated in the \toolname{} model to get superior runtime performance.

%So, similar to \emph{VERSE}, we introduce a negative sampling based repulsive force calculation which is described in the next section.

\begin{algorithm}[!ht]
\caption{Negative Sampling based Force2Vec Algorithm}\label{euclid}
\begin{flushleft}
\textbf{Input:} G(V, E) and an initial embedding $z$\\
\textbf{Output:} optimized embedding of $z$
\end{flushleft}
\begin{algorithmic}[1]
\State $\eta = 0.02$ \Comment{initial learning rate}
\State $c = 0$ \Comment{initialize loop counter}
\While {$ c < Max$}
    \State $f = 0$ \Comment{force initialization}
    \For{$b \leftarrow$ 0 to $\frac{n}{B}-1$}
        \For{$i\leftarrow$ 0 to $s-1$}
            \State $randi \leftarrow $ random index from $[0\ldots n-1]$
            \State $z'_i = z_{randi}$
        \EndFor
        \For{$u \leftarrow b\times B$ to $(b+1)\times B -1$}
            \For{$v \in N(v)$}
                \State $f_u = f_u + \nabla f_a(z_u,z_v)$%\times \frac{z_u - z_v}{\parallel z_u - z_v\parallel}$
            \EndFor
            \For{$v \leftarrow 0$ to $s-1$}
                \State $f_u = f_u + \nabla f_r(z_u,z'_v)$%\times \frac{z_u - z'_v}{\parallel z_u - z'_v\parallel}$
            \EndFor
        \EndFor
        \For{$u \leftarrow b\times B$ to $(b+1)\times B -1$}
            \State $z_u = z_u - \eta \times f_u$
        \EndFor
    \EndFor
    %\State $\eta = 1 - \frac{c}{Max}$
    %\State $\eta = 0.999\times \eta$
    \State $c = c + 1$
\EndWhile
\State \Return the final embedding $z$
\end{algorithmic}
\label{algo:nsforce2vecalgo}
\end{algorithm}

Algorithm \ref{algo:nsforce2vecalgo} performs well for homogeneous networks as it considers only neighboring vertices for \emph{attractive} force calculations, but, intuitively, it can not capture enough information from heterogeneous networks. Thus, to capture more information from heterogeneous networks, we introduce a variation which is based on semi-random walks. In this approach, for each vertex $u$, we select a $walklength$ number of vertices from its subsequent $k$-hop neighbors $N_k(u)$ for calculating \emph{attractive} forces. This approach facilitates each vertex $u$ to directly interact with its $k$-hop neighbors to capture structural information. We formally present this approach in Algorithm \ref{algo:nsforce2vecalgorw}. Note that, we only insert lines 5 to 11 for selecting neighbors for each vertex of the graph $G$ and keep everything else similar to Algorithm \ref{algo:nsforce2vecalgo}. Asymptotic runtime and memory consumption of Algorithm \ref{algo:nsforce2vecalgorw} remains the same as Algorithm \ref{algo:nsforce2vecalgo}.

\begin{algorithm}[!ht]
\caption{Semi-random Walk based Force2Vec Algorithm}\label{euclid}
\begin{flushleft}
\textbf{Input:} G(V, E) and an initial embedding $z$\\
\textbf{Output:} optimized embedding of $z$
\end{flushleft}
\begin{algorithmic}[1]
\State $\eta = 0.02$ \Comment{initial learning rate}
\State $c = 0$ \Comment{initialize loop counter}
\While {$ c < Max$}
    \State $f = 0$ \Comment{force initialization}
    \For{$u\leftarrow$ 0 to $n-1$}
        \State $v \leftarrow 0$ 
        \State $j \leftarrow u$
        \While{$v < walklength-1$}
            \State $W_{uv} \leftarrow $ random vertex from $N(j)$
            \State $j \leftarrow W_{uv}$
            \State $v = v + 1$
        \EndWhile
    \EndFor
    \For{$i\leftarrow$ 0 to $s-1$}
        \State $randi \leftarrow $ random index from $[0\ldots n-1]$
        \State $z'_i = z_{randi}$
    \EndFor
    \For{$b \leftarrow$ 0 to $\frac{n}{B}-1$}
        \For{$u \leftarrow b\times B$ to $(b+1)\times B -1$}
            \For{$v \in W_u$}
                \State $f_u = f_u + \nabla f_a(z_u,z_v)$
            \EndFor
            \For{$v \leftarrow 0$ to $s-1$}
                \State $f_u = f_u + \nabla f_r(z_u,z'_v)$
            \EndFor
        \EndFor
        \For{$u \leftarrow b\times B$ to $(b+1)\times B -1$}
            \State $z_u = z_u - \eta \times f_u$
        \EndFor
    \EndFor
    %\State $\eta = 1 - \frac{c}{Max}$
    %\State $\eta = 0.999\times \eta$
    \State $c = c + 1$
\EndWhile
\State \Return the final embedding $z$
\end{algorithmic}
\label{algo:nsforce2vecalgorw}
\end{algorithm}

\subsection{Preliminary Results}
\begin{table*}[!ht]
\centering
\caption{Runtimes (sec.) taken by different tools to generate embeddings for corresponding datasets using 48 threads. \toolname{} represents runtime of Algorithm \ref{algo:nsforce2vecalgo} with $t$-distribution. Number in parenthesis represents approximate speedup of \toolname{}.}
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Methods}  & {\color[HTML]{333333} \textbf{DeepWalk}} & {\color[HTML]{333333} \textbf{LINE}} & {\color[HTML]{333333} \textbf{struc2vec}} & {\color[HTML]{333333} \textbf{Verse}} & {\color[HTML]{333333} \textbf{Force2Vec}} \\ \hline
\textbf{Cora}     & 73.95 ($\approx$52$\times$)                     & 1913.29 ($\approx$1347$\times$)             & 274.52 ($\approx$193$\times$)                    & 46.99 ($\approx$33$\times$)                  & 1.42                                          \\ \hline
\textbf{Citeseer} & 87.24 ($\approx$53$\times$)                     & 1889.01 ($\approx$1152$\times$)             & 367.05 ($\approx$224$\times$)                    & 55.94 ($\approx$34$\times$)                  & 1.64                                          \\ \hline
\textbf{Pubmed}   & 591.48 ($\approx$54$\times$)                    & 1897.5 ($\approx$173$\times$)               & 2199.16 ($\approx$200$\times$)                   & 300.35 ($\approx$27$\times$)                 & 10.98                                         \\ \hline
\textbf{Flickr7}  & 1989.56 ($\approx$38$\times$)                   & 10259.28 ($\approx$195$\times$)             & 8176.75 ($\approx$156$\times$)                   & 1297.92 ($\approx$25$\times$)                & 52.52 \\ \hline
\textbf{Youtube}  & 28049.52 ($\approx$58$\times$)                  & 12843.44 ($\approx$27$\times$)              & x                                         & 15798.77 ($\approx$33$\times$)               & 480                                         \\ \hline
\end{tabular}
\label{tab:runtimes}
\end{table*}

To compare the effectiveness of our proposed method with respect to existing techniques, we develop a C++ tool using Algorithm \ref{algo:nsforce2vecalgo} with $t$-distribution based optimization in shared memory parallel environment. We also conduct experiments in small scale. We provide running time of \toolname{} in Table \ref{tab:runtimes} along with other state-of-the-art methods. In particular, for the largest dataset (Youtube), \toolname{} is 58$\times$, 27$\times$ and 33$\times$ faster than \deepwalk{}, \linet{} and \verset{}, respectively. Note that, \linet{} is significantly slower for comparatively small graphs due to asynchronous thread usage and optimization. Sometimes, this huge running time is introduced by \emph{false sharing}, a common phenomena in shared memory parallelism caused by asynchronously dependent read-write operations in memory \cite{bolosky1993false}. We avoid this dependency by employing batch processing of vertices (see Fig. \ref{fig:batchforce}) and thus, improve the performance. Because of the huge running time cost of \structtwovec{}, we could not produce results for the Youtube dataset within the imposed 40 hours time limit.

\begin{figure}
    \centering
    \includegraphics[width=0.42\linewidth]{figures/citeseerclassification.pdf}
    \includegraphics[width=0.42\linewidth]{figures/pubmedclassification.pdf}
    \caption{F1-micro scores for classification task on (a) Citeseer and (b) Pubmed datasets.}
    \label{fig:force2vecclassification}
\end{figure}

In Fig. \ref{fig:force2vecclassification}, we report the results for the classification task on the Citeseer and Pubmed datasets. We observe that the embedding generated by Algorithm \ref{algo:nsforce2vecalgo} with $t$-distribution performs better than other methods for the Citeseer dataset (see Fig. \ref{fig:force2vecclassification} (a)). For the Pubmed dataset (see Fig. \ref{fig:force2vecclassification} (b)), both \toolname{} and \deepwalk{} perform equally well compared to other methods. Thus, our preliminary results show that \toolname{} can generate high quality embeddings faster than other methods and perform as well or better in different downstream prediction tasks.

\section{Future Directions}
\label{sec:futuredir}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/simdvectorization.png}
    \caption{An example of (a) general and (b) SIMD vector addition.}
    \vspace{-0.3cm}
    \label{fig:simdfigure}
\end{figure}
\subsection{Scalability}
\subsubsection{SIMD Vectoization}
Single Instruction Multiple Data (SIMD) is a strategy in parallel computing that transforms the data elements in a packed one dimensional array by performing one arithmetic operation on the packed elements at once. We can explain this technique by Fig. \ref{fig:simdfigure}. When we perform an addition operation on an array of elements (see Fig. \ref{fig:simdfigure} (a)), we generally iterate over the array and execute the addition operation one by one. For example, to execute $e[i] = a[i] + c[i]$ without optimization in C++, the processor performs addition on arrays $a$ and $c$ one by one i.e., add the first elements of $a$ and $c$, then store it back in the first position of $e$; after this, it picks the second elements of $a$ and $c$, performs addition and store it back to the second position of $e$ and so on. However, with SIMD support (see Fig. \ref{fig:simdfigure} (b)), the processor can perform one single addition operation on a packed array of 8 or 16 elements. For example, a SIMD supported processor can execute the statement $e[i] = a[i] + c[i]$ for 8 or 16 consecutive elements at a time, thus, increasing the speed-up. In an \textbf{$\mathbf{AVX512}$} supported machine, the processor can perform 16 parallel additions on 4-bytes integer array elements.

In the straightforward implementation of calculating forces from an adjacency matrix, we can not avoid conditional statements to determine whether two vertices are neighbors or not. These conditional statements are not friendly for SIMD vectorization. In the Compressed Sparse Row (CSR) representation of a graph, we easily find neighbors of a vertex from \emph{colids}, which is helpful to calculate the attractive force without any conditional statements. We then use the SIMD directive of OpenMP to vectorize our algorithms. This type of vectorization solely depends on the compiler based on several optimization flags. So, without depending on a compiler, we can further optimize our algorithms using \textbf{$\mathbf{AVX512}$} \emph{intrinsic} instruction sets available in a Skylake server machine to make it fully vectorized. This will optimize running time for every single core in the server machine.

\subsubsection{Distributed System}
With the advancement of technologies, we are producing huge amounts of data\footnote{It has been predicted that the Global Datasphere could grow up to 175 ZettaBytes (ZB) by 2025 \cite{reinsel2018digitization}} at an increasing velocity by social interactions. For such large, real-world social graphs, such as the facebook network, having billions of nodes, we can not fulfil memory requirement in a single machine for efficient computations. Therefore, we need to employ computations in distributed systems. Once we have optimized the method for single core machines using SIMD vectorization, we will focus on distributed algorithms that preserve the quality of the embedding and accelerate computation. As a high level overview, we will perform the following set of tasks to accomplish our goal:

\begin{itemize}
    \item We will distribute disk I/O operations across all machines in the cluster. We intend to use the C++ OpenMPI library for developing our distributed algorithm for \toolname{}. In particular, we will use $\mathbf{MPI\_File\_read\_at}$ and $\mathbf{MPI\_File\_write\_at}$ with the necessary helper functions available in the MPI library for parallel I/O operations.
    \item We will disseminate force computations across all machines in the cluster using distributed minibatch processing. We will further parallelize computations in a single machine using multi-threaded programming in appropriate scenarios. This step will heavily depend on the size of the graph, e.g., small graph can be processed faster in a multi-threaded single machine as opposed to distributed machines. 
    \item Most real-world networks are sparse. Thus, there is a little reuse of data for computations. So, our approach will be memory bounded. We will use a cache blocking technique to optimize the bandwidth utilization by reducing back and forth data movement for memory read/write operations. A significant portion of total running time in distributed systems comes from the communication cost over the network. In our distributed \toolname{} framework, we will focus on employing communication-avoiding \cite{koanantakool2017communication} and synchronization-avoiding \cite{firoz2018synchronization} strategies.
\end{itemize}

\subsection{Domain Specific Graph Learning}
Once we have a distributed framework for graph representation learning, various graph embedding problems can be formulated in our model easily. At this stage, we will focus on developing a model for transitive path prediction for directed graphs and incorporating domain specific features in graph embedding. In our previous discussion, we have seen that unsupervised graph embedding methods do not employ domain specific features while learning representations from a graph. One naive, but baseline, idea can be to concatenate domain specific features with the output embedding of a graph. However, its effectiveness totally depends upon the quality of the extracted information from the corresponding domain. On the other hand, a GCN can take domain specific features in the input layer and show better performance in the node classification task. So, we will work on developing a scalable distributed GCN framework for domain specific applications.

\subsection{Visualization and Interpretability}
 Graph visualization has been explored widely in the literature. As most real-world networks change over time, their inherent information is dynamic in nature. A straight-forward way to visualize such graphs is to generate the layout again with respect to changes in the network, which is an inefficient approach. Efforts have been made to visualize such dynamic graphs though, sometimes, it is hard to find meaningful information from its representation, especially when the size of the graph is large \cite{burch2011parallel,beck2017taxonomy}. Graph Convolutional Networks (GCN) can help us to visualize dynamic graph in an \emph{inductive} way. The basic idea can be formulated in the following way: (i) Firstly, we cluster the graph using Louvain algorithm and consider the cluster identifier as the label of each vertex. (ii) Secondly, we train a GCN to generate a layout of the graph for visualization from the initial structure. This step learns weights for different layers of the GCN. (iii) Thirdly, when new nodes arrive in the network, we generate layouts for them using the already learned weights of the GCN and associated neighbors. (iv) Finally, we update the weights of the GCN after the arrival of a certain number of new nodes. Sometimes, the visualization of intermediate layers in Convolutional Neural Networks (CNN) can reveal some inherent information, such as types of features extracted from images, e.g., a convolutional layer in CNN can detect edges in the image \cite{zeiler2014visualizing}. Finally, being motivated by this work, we will focus on employing similar interpretability of hidden layers in a GCN.
 
 
 
\begin{comment}
\begin{table}[!ht]
\centering
\begin{tabular}{l|c|c|c|c|c|c|c|}
\cline{2-8}
\multicolumn{1}{c|}{}                  & \multicolumn{7}{c|}{\textbf{Runtime in seconds for different graphs}}                                                        \\ \hline
\multicolumn{1}{|c|}{\textbf{Methods}}& \textbf{PPI} & \textbf{Cora}  & \textbf{Citeseer} & \textbf{Pubmed} & \textbf{Flickr7} & \textbf{BlogCatalog} & \textbf{Youtube}  \\ \hline
\multicolumn{1}{|l|}{\structtwovec{}} &  157.26    & 274.52         & 367.05            & 2199.16         & 8176.75  & -         & -                 \\ \hline
\multicolumn{1}{|l|}{\verset{}}  &   \textbf{44.65}       & \textbf{46.99} & \textbf{55.94}    & \textbf{300.35} & \textbf{1297.92} & \textbf{158.04} & 15798.77          \\ \hline
\multicolumn{1}{|l|}{\linet{}}  &     \textcolor{red}{16182.44}      & 1913.29        & 1889.01           & 1897.5          & 10259.28  & 11495.6       & \textbf{12843.44} \\ \hline
\multicolumn{1}{|l|}{\deepwalk{}} &  49.614      & 73.95          & 87.24             & 591.48          & 1989.57  & 332.296    & 28049.53          \\ \hline
\end{tabular}
\caption{Runtime (in seconds) of different shallow network based tools for different benchmark graphs. We run all tools using same computing resources. Better runtime is shown in bold face for each dataset.}
\label{tab:runtimegraphs}
\end{table}
\end{comment}


\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{figures/results/aMulti-labelclassificationononPPI.pdf}
    \includegraphics[width=0.4\linewidth]{figures/results/bMulti-labelclassificationononPPI.pdf}
    \caption{Results of (a) F1-micro scores and (b) F1-macro scores on multi-label classification task for PPI graph}
    \label{fig:abppimultilabel}
\end{figure}


%**********************************
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10010147.10010169.10010170.10010171</concept_id>
       <concept_desc>Computing methodologies~Shared memory algorithms</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10003120.10003145.10003146.10010892</concept_id>
       <concept_desc>Human-centered computing~Graph drawings</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10002951.10003260.10003261.10003270</concept_id>
       <concept_desc>Information systems~Social recommendation</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010258.10010260.10010271</concept_id>
       <concept_desc>Computing methodologies~Dimensionality reduction and manifold learning</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010257.10010258.10010260.10003697</concept_id>
       <concept_desc>Computing methodologies~Cluster analysis</concept_desc>
       <concept_significance>500</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Shared memory algorithms}
\ccsdesc[300]{Human-centered computing~Graph drawings}
\ccsdesc[500]{Information systems~Social recommendation}
\ccsdesc[500]{Computing methodologies~Dimensionality reduction and manifold learning}
\ccsdesc[500]{Computing methodologies~Cluster analysis}

\hyphenation{op-tical net-works semi-conduc-tor}
%******************************

